Modeling and Analyzing Scorer Preferences in Short-Answer Math Questions

Automated scoring of student responses to open-ended questions, including short-answer questions, has great potential to scale to a large number of responses. Recent approaches for automated scoring rely on supervised learning, i.e., training classifiers or fine-tuning language models on a small number of responses with human-provided score labels. However, since scoring is a subjective process, these human scores are noisy and can be highly variable, depending on the scorer. In this paper, we investigate a collection of models that account for the individual preferences and tendencies of each human scorer in the automated scoring task. We apply these models to a short-answer math response dataset where each response is scored (often differently) by multiple different human scorers. We conduct quantitative experiments to show that our scorer models lead to improved automated scoring accuracy. We also conduct quantitative experiments and case studies to analyze the individual preferences and tendencies of scorers. We found that scorers can be grouped into several obvious clusters, with each cluster having distinct features, and analyzed them in detail.

==> analysis.tex <==
\section{Qualitative Analysis} 
\subsection{Scalar bias and variance with scorer embeddings}
%\subsection{Analysis $b_{c,j}$ and $\alpha_j$}
We now qualitatively analyze the trained model that uses scorer embeddings to characterize the individual bias and variance of each scorer (detailed in Sec.~\ref{sec:semb}). 

\subsubsection{Visualization of scorer embedding}
Figure~\ref{fig:emb_bcj} shows a 2-D visualization of the learned scorer embedding space; We see that there are obvious clusters among all scorers. We then fit the learned scorer embeddings under a mixture-of-Gaussian model via the expectation-maximization (EM) algorithm with $6$ clusters. The subfigures to each side of the main plot show each cluster's average bias towards each score category, which are $0$, $1$, $2$, $3$, and $4$ from left to right. 

% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth, height=0.6\textwidth]{figures/visulization1.png}
%     \caption{\ml{needs to be remade - central figure smaller, the side ones larger (y-axis label: bias), font size also larger, change the cluster labels to from 1 to 6. subfigure titles should be cluster x. y axis should be bias. need to explain in the caption or main text what does each dot and each circle/shaded area mean. otherwise pretty good}}
%     \label{fig:emb_bcj}
% \end{figure}
\begin{figure*}%
    \centering
    \subfloat[\centering 2-D visualization of the learned scorer embedding space ]{{\includegraphics[width=0.5\textwidth]{figures/cluster_b_alpha.png}}}%
    %\qquad
    \hspace{-.5cm}
    \subfloat[\centering Bias for each score category]{{\includegraphics[width=0.5\textwidth]{figures/bias.png}}}%
    \caption{Visualization of clustering result on scorer embedding learnt via scorer-specific model. The left figure shows the 2-D visualization of scorer embedding space and the right figure shows the average bias for each cluster}%
    \label{fig:emb_bcj}%
\end{figure*}

\begin{table}[ht]  
  \scalebox{.8}{
  \begin{tabular}
      %{lllll}
      %{p{0.1\textwidth}>{\centering}|p{0.2\textwidth}>{\centering}p{0.2\textwidth}>{\centering\arraybackslash}p{0.2\textwidth}>{\centering}p{0.2\textwidth}>{\centering}}
      {M{0.08\textwidth}|
      M{0.15\textwidth} %figure bias 
      M{0.15\textwidth} %figure  groundtruth
      M{0.1\textwidth} %temperature
      M{0.1\textwidth} %
      M{0.1\textwidth}
      M{0.1\textwidth}
      M{0.1\textwidth}}
      
      \hline 
      Cluster & 
      Bias & 
      Observed scoring distribution (normalized) & 
      Temperature & 
      Score  & 
      \multicolumn{3}{c}{Response features}
      \\\cline{6-8}
       &&&&&math tok (\%)&img (\%)&length\\
      
      \hline
      1
      & \parbox[l]{0.15\textwidth}{\includegraphics[width=0.15\textwidth]{figures/cluster0.png}} 
      &\parbox[l]{0.15\textwidth}{\includegraphics[width=0.15\textwidth]{figures/groun_truth0.png}} 
      & 1.013%alpha 
      &  1.685 $\pm$ 1.644 % gradeing 
      & 29.13 %math tok 
      & 0.101 %img
      & 23.06%length 
      \\
      \hline
      2
      & \parbox[l]{0.15\textwidth}{\includegraphics[width=0.15\textwidth]{figures/cluster1.png}} 
      &\parbox[l]{0.15\textwidth}{\includegraphics[width=0.15\textwidth]{figures/groun_truth1.png}} 
      & 1.034%alpha 
      &  3.451 $\pm$ 0.919% gradeing 
      & 32.12 %math tok 
      & 1.286%img
      & 24.40%length
      \\
      \hline
      3
      & \parbox[l]{0.15\textwidth}{\includegraphics[width=0.15\textwidth]{figures/cluster2.png}} 
      &\parbox[l]{0.15\textwidth}{\includegraphics[width=0.15\textwidth]{figures/groun_truth2.png}} 
      & 0.996%alpha 
      &  2.415 $\pm$ 1.400 % gradeing 
      & 23.51 %math tok 
      & 1.311%img
      & 36.16%length 
      \\
      \hline
            4
      & \parbox[l]{0.15\textwidth}{\includegraphics[width=0.15\textwidth]{figures/cluster3.png}} 
      &\parbox[l]{0.15\textwidth}{\includegraphics[width=0.15\textwidth]{figures/groun_truth3.png}} 
      & 1.033%alpha 
      &  3.074 $\pm$ 0.991 % gradeing 
      & 29.48 %math tok 
      & 0.304%img
      & 21.94%length 
      \\
      \hline
            5
      & \parbox[l]{0.15\textwidth}{\includegraphics[width=0.15\textwidth]{figures/cluster4.png}} 
      &\parbox[l]{0.15\textwidth}{\includegraphics[width=0.15\textwidth]{figures/groun_truth4.png}} 
      & 1.026%alpha 
      &  2.558 $\pm$ 1.806% gradeing 
      & 45.18%math tok 
      & 5.271%img
      & 14.35%length 
      \\
      \hline
      6
      & \parbox[l]{0.15\textwidth}{\includegraphics[width=0.15\textwidth]{figures/cluster5.png}} 
      &\parbox[l]{0.15\textwidth}{\includegraphics[width=0.15\textwidth]{figures/groun_truth5.png}} 
      & 1.007%alpha 
      &  2.714 $\pm$ 1.331% gradeing 
      & 33.83 %math tok 
      & 1.403%img
      & 13.34%length 
      \\
      \hline
  \end{tabular}}
  \vspace{.2cm}
  \caption{Detailed biases and variance (inverse of temperature) for each scorer profile, their observed scoring distributions, and average response features. We normalize the observed scoring distributions to zero-mean, which makes them easier to visually compare against the learned biases. \textit{math tok (\%)} is the percentage of math tokens in the response. \textit{img (\%)} is the percentage of image in the response. \textit{length} is the number of word tokens in the response.}
  \label{tab:bcj}
\end{table}
\subsubsection{Features analysis base on each cluster}
%The average bias scores of cluster 0 indicate that teachers in this cluster are prone to give 0. 
Cluster $1$ shows a negative scoring profile, with a strong, positive bias towards the lowest sore category $0$ (positive $b_{c,j}$ values) and small, negative biases against higher scores, $1$, $2$, and $3$ (negative $b_{c,j}$ values). These scorers assign $0$ scores much more often than other score categories, compared to other scorers. The average score across question-response pairs is the lowest for this cluster, at $1.69$. Meanwhile, this cluster has a relatively high score variance of $1.69$, meaning that these scorers tend to have inconsistent behavior and assign a wide variety of score labels. 

%s (1, 2, 3, and 4) all have some negative biases, similar to what has been shown in the ground truth: there are apparently more zeros than other scores, and numbers of 1, 2, 3, and 4 are lower than the average. The main difference is that the bias of 4 is slightly lower than the ground truth, which is also shown in Table 1. We can see that teachers in this cluster give the lowest average grade of 1.69. However, the variance, 1.69, is relatively high, meaning that the range of scores these teachers grade is extensive, but most scores are low.  

Cluster $2$ shows a positive scoring profile, with a strong, positive bias towards the highest score, $4$ and moderate negative biases against other scores. These scorers prefer to assign scores that are overwhelmingly higher compared to other scorers. The average score across question-response pairs is the lowest for this cluster, at $3.45$. Meanwhile, this cluster has a relatively low score variance of $0.92$, meaning that these scorers are consistent in scoring responses higher than other scorers.  

Cluster $3$ shows a conservative scoring profile, with small, positive biases towards the middling scores $1$, $2$, and $3$ and a strong, negative bias against the top score $4$. The average score across question-response pairs is $2.41$ for this cluster with a variance of $1.4$, which is high considering that scorers in this cluster rarely use the top score category, indicating that their scoring behavior is not highly consistent. 

Cluster $4$ shows an unbiased scoring profile, with low bias towards or against any score category, with a slight preference for the top score category, $4$. This cluster contains almost half of the scorers, which means that the majority of scorers are reliable (their scores depend mostly on the actual quality of the response, i.e., the $\mathbf{w}_c^T \mathbf{r}_i$ term in Eq.~\ref{eq:scalar} rather than the bias term. 

Cluster $5$ shows a polarizing scoring profile, with strong, positive biases toward both the lowest score, $0$, and the highest score, $4$, while having strong, negative biases against score categories in between. Scorers in this cluster often score a response as all or nothing, while using the intermediate score values sparingly. The average score across question-response pairs is $2.55$ for this cluster with a variance of $1.81$, the highest among all clusters, which agrees with our observation that these scorers are highly polarizing and rarely judge any response to be partially correct. 

Cluster $6$ shows a lenient scoring profile, with a strong, negative bias against the lowest score, $0$, and a moderate, positive bias towards the next score, $1$, with minimal bias across higher score categories. Scorers in this cluster tend to award students a single point for an incorrect response instead of no points at all. The average score across question-response pairs is $2.71$ for this cluster with a middling variance of $1.33$. 



\subsubsection{Correlation analysis}
\begin{figure}%
    \centering
    \subfloat[\centering Correlation Coefficient Matrix]{{\includegraphics[width=0.5\textwidth]{figures/corre1.png}}}%
    %\qquad
    \hspace{-.5cm}
    \subfloat[\centering P-values Matrix]{{\includegraphics[width=0.5\textwidth]{figures/pvalue1.png}}}%
    \caption{Correlation coefficients and corresponding p-values across the bias, variance terms, and response features for the scorer-specific bias and variance models.}%
    \label{fig:corrp1}%
\end{figure}

In Table~\ref{tab:bcj}, we see that the learned scorer biases for each cluster are highly correlated with the observed score distribution across score categories. However, it is not obvious how the variance, i.e., the inverse of the temperature parameter ($\alpha$), correlates with other model parameters and response features. Therefore, we calculate the correlation coefficient (left) and the corresponding p-value (right) between each pair of model parameter and response features and show them in Figure~\ref{fig:corrp1}. In the left part of the figure, we see that $\alpha$ positively correlates with the mean of scores and negatively correlates with the standard deviation of scores. In the right part of the figure, we see that $\alpha$ is significantly correlated with the standard deviation of scores, which is as expected since this temperature parameter is designed to capture the variation in score category assignments. We also see that $\alpha$ is also significantly correlated with the bias terms of each score category, with a positive correlation with the bias for score category $4$ and negative correlation with the bias for other categories.  

For the bias terms, we see that most of the biases are significantly correlated with the mean and standard deviation of scores, but less correlated with question-response pair features. This observation suggests that the bias terms mainly depend on scorer behavior rather than the question-response pair, which is what the model intended to do; the question-response pair is captured by the $\mathbf{w}_c^T \mathbf{r}_i$ term in Eq.~\ref{eq:scalar}. The bias for score category $2$, however, does not significantly correlate with the mean and standard deviation of scores but significantly correlates with other question-response pair features. One possible explanation is that since this score category is the middle of all scores, scorers do not show any bias towards or against this score category and can solely rely on the actual content of the question and response. 
%, for example the length of the response which might shows that bias 2 does not accurately represent scorer grading behavior.   

%\subsubsection{Case study}

\subsection{Content-driven scorer bias and variance: case study}
\subsubsection{Visualization of scorer embedding}
\begin{figure}
    \centering
    \includegraphics[width=.6\textwidth]{figures/cluster_b_alpha5.png}
    \caption{Scorer embeddings learned via the content-driven scorer bias and variance model. Different from the scorer-specific bias and variance case, these embeddings are not clearly grouped into clusters.}
    \label{fig:emb_bc_clsj}
\end{figure}

Figure~\ref{fig:emb_bc_clsj} shows the 2-D visualization of the scorer embeddings learned under the content-driven scorer bias and variance model. 
We see that the sorcerer embedding are widely spread across the embedding space with no obvious clusters after running the same EM algorithm as above. One possible explanation is that under the content-driven scorer bias and variance setting, the scorer embedding encodes not only scorer preferences and tendencies but also how they process the textual information in question-response pairs. Therefore, one cannot isolate out the impact of biases and variances from the content-driven term in the scoring model, $\mathbf{w}_c^T \mathbf{r}_i$. However, we do see that the learned bias and variance parameters match the overall trend of the observed score distributions, which means that the bias and variance parameters still help the model to fit better to the data, at the expense of losing interpretability. 



\begin{figure}%
    \centering
    \subfloat[\centering Correlation Coefficient Matrix]{{\includegraphics[width=0.5\textwidth]{figures/corre5.png} }}%
    \hspace{-.5cm}
    \subfloat[\centering P-values Matrix]{{\includegraphics[width=0.5\textwidth]{figures/pvalue5.png} }}%
    \caption{Correlation coefficients and corresponding p-values across the bias, variance terms, and response features for the content-driven bias and variance models.}%
    \label{fig:corr_content}%
\end{figure}
\subsubsection{Correlation analysis}

Figure~\ref{fig:corr_content} shows the correlation coefficient and corresponding p-value matrices for the content-driven scorer bias and variance models. Comparing it to the scorer-specific bias and variance models in Figure~\ref{fig:corrp1}, we can see that temperature/inverse variance parameter $\alpha$ and bias have a stronger correlation with question-response pair features, which is expected since these parameters depend on the textual representation of questions and responses in this model. One interesting observation is that $\alpha$ only correlates with the mean of scores and no longer correlates with the standard deviation of scores. Correlation between the biases of different score categories also decreases significantly compared to the scorer-specific model. This result may suggest that the model learns more meaningful biases as a function of $\mathbf{r}_i$. In addition, this result explains why content-driven scorer models have higher RMSEs (higher is worse) than scorer-specific models but also higher Kappa and AUC values (higher is better). It may also explain why the RMSE values across all models are similar.

\begin{table}[]
\scalebox{.6}{
\begin{tabularx}{\textwidth}{|l|X|l|l|l|l|l|}
\hline
Question& Response & Actual & Content- & Scorer- & No & Content-driven scorer bias                                   \\
id & &  score&  driven & specific &  bias &  \\
 & &  &  prediction & prediction &  prediction &  \\

\hline
1    & The graph was touching the origin, but it didn't have a straight line         & 4          & 4                      & 4                       & 3               & {[}-0.61, -1.29, 0.04, -0.33, 1.33{]}  \\ \hline
2     & It meets the origin and it goes perfectly diagonal.                           & 3          & 4                      & 4                       & 3               & {[}-0.26, -1.80, -0.57, -0.39, 2.09{]} \\ \hline
            & Because it's a straight line that goes through the orgin                      & 4          & 4                      & 4                       & 3               & {[}0.13, -1.53, -0.76, -0.47, 1.71{]}  \\ \hline
            & its porportional because it has a straight line and and starts at the bottom. & 3          & 3                      & 4                       & 2               & {[}1.19, -0.20, -3.18, 1.24, 1.21{]}   \\ \hline
            & idk                                                                           & 3          & 3                      & 0                       & 0               & {[}-6.26, -0.09, 2.76, 4.56, 1.50{]}   \\ \hline
%3     & They are not proportional because the line is not straight.                   & 2          & 2                      & 4                       & 0               & {[}-0.77, -0.59, 0.16, 0.36, 0.40{]}   \\ \hline
%            & it isn't proportional because the lines go up and then to the side            & 2          & 4                      & 4                       & 4               & {[}-0.41, -1.18, -0.18, -0.28, 1.18{]} \\ \hline
%            & they dont meet the orgin                                                      & 4          & 4                      & 4                       & 4               & {[}0.40, -0.54, -0.49, -1.06, 0.57{]}  \\ \hline
\end{tabularx}}
\vspace{.2cm}
\caption{Examples of student response and scores for a single scorer with biases $-0.043, -0.36, 0.061, -0.212, 0.439$ for all score categories. Notice that the no-bias prediction is the prediction of the content-driven model that does not scale with bias.}
\label{tab:case1}
\end{table}



\subsection{Case study: same scorer, different responses}
%\subsubsubsection{Same scorer grading different question}

Table~\ref{tab:case1} shows several examples of different questions and responses and corresponding scores for a single scorer, with the actual score, biases calculated from the content-driven scorer bias and variance model, and predicted scores for different models. The overall bias for this scorer is $-0.043, -0.36, -0.212, 0.061, 0.439$ across all score categories, which indicates that this scorer prefers to assign high scores (especially the full score $4$) but often assigns low scores except the lowest score ($0$). Overall, we see that if we do not include biases into the AS model (the sixth column), the AS model tend to predict middling scores, while the human scorer tend to give students full credit ($4$). For Question~2, this example shows that the content-driven scorer bias model captures nuanced scorer preference: for the meaningless response ``idk'', which should have a score of $0$, the scorer has a strong preference towards giving it a high score ($3$). This bias only appears for seemingly meaningless responses but not overall (overall bias towards score category $3$ is minimal at $0.061$). Therefore, we see that the scorer-specific model cannot capture this information since its biases and variance are global across all question-response pairs for this scorer. As a result, content-driven scorer models are more flexible in handling these cases compared to other models, which is also evident in the quantitative results in Table~\ref{tab:as} that this model achieves the highest overall AS accuracy. 
%As we can see each content scorer bias is different more or less to others. It also has the trend increase weight on score 4 but the scope is various. scorer specific predict only predict value 4 or 0 where content scorer model can predicts more accurate. One interesting result shows in question id: 1057712 and response: idk. It should be scored as 0 credit for sure, but the the content-scorer predicts result as 3.

==> result.tex <==
\section{Quantitative Experiments}

We now detail experiments that we conducted to validate the different scoring components of AS models and loss functions that capture scorer preferences and tendencies. Section~\ref{sec:data} discusses details on the real-world student response dataset we use and the pre-processing steps. Section~\ref{metrics} details the evaluation metrics we use in our experiments. Section~\ref{setting} details our experimental setting and Section~\ref{result} details the experimental results and corresponding discussion. 

\subsection{Dataset}
\label{sec:data}

We use data collected from an online learning platform that has been used in prior work~\cite{sami,erickson}, which contains student responses to open-ended, short-answer math questions, together with scores assigned by human scores. 
%The dataset was originally collected with student answers to open response question in the ASSISTments \cite{assist} online learning platform. 
There are a total of 141,612 total student responses made by $25,069$ students to $2,042$ questions, with $891$ different teachers are scorers. The set of possible score categories is from $0$ (no credit) to $4$ (full credit). The dataset mainly contains math word problems, where the answer could be mathematical such as numbers and equations or textual explanations, sometimes in the format of images. %In this dataset, some same or similar response-question pairs may have different grades due to various scorers. For this study our focus is on exploring weather modeling grader behavior is helpful for AS task, thus this dataset fits in our purpose well.

We found that different scorers sometimes assign very different scores to the same response, which motivated this work. As an example, we analyze question-response pairs that are scored by more than one scorer and evaluate the Kappa score between these scorers. The \emph{human} Kappa score is only $0.083$, which means a minimal agreement between different scorers. Although there are only $523$ such pairs, this case study still shows that even for the same exact response, scorers have highly different individual preferences and tendencies and may assign them highly different scores. 

We also perform a series of pre-processing steps to the original dataset. For example, since some of the scorers do not score many responses, e.g., less than $100$, there many not be enough information on these scorers for us to model their behavior. Therefore, we remove these scores from the dataset, which results in $203$ scorers, $1,273$ questions and $118,079$ responses. The average score is $3.152 \pm 1.417$. Table~\ref{tab:example} shows some examples data points of this dataset; each data point consists of the question statement, the student's response, the scorer's ID, and the score. 

\begin{table*}[h]
\resizebox{2\columnwidth}{!}{
\begin{tabularx}{\textwidth}{ l|X|X|l|l }
  \toprule
  $question\_id$ & $question\_body$  & $response$  & $scorer\_id$ & $score$ \\ \hline
  43737 & Chris spent \$9 of the \$12 he was given for his birthday. His sister Jessie says that he has spent exactly 0.75 of the money. Chris wonders if Jessie is correct. Explain your reasoning. & 
  Jessie is correct because 0.75 in fraction form is 3/4. 9 is 3/4 of 12, so she is right. & 1 &4 \\
  \cline{3-5}
  && Jessie is wrong. & 1 & 0\\
\cline{3-5}
  && she is correct & 1&1 \\
  \cline{3-5}
  && Jessie is incorrect.& 2 & 4 \\ 
  \cline{3-5} 
  && Jessie is right because if you divide 12 by 9 you get 0.75. & 2 & 2\\
  \bottomrule
\end{tabularx}}
\vspace{.2cm}
\caption{Example questions, student responses, and scores. Some scorers assign highly different scores to similar responses.}
\label{tab:example}
\end{table*}


\subsection{Metrics}
\label{metrics}
We utilize three standard evaluation metrics for integer-valued scores that have been commonly used in the AS task \cite{sami,erickson}. First, the area under the receiver operating characteristic curve (\textbf{AUC}) metric, which we adapt to the multi-category classification problem by averaging the AUC numbers over each possible score category and treating them as separate binary classification problems, following \cite{hand2001simple}. Second, we use the root mean squared error (\textbf{RMSE}) metric, which simply treats the integer-valued score categories as numbers, as detailed in Eq.~\ref{eq:mse}. Third and most importantly, we use the multi-class Cohen's \textbf{Kappa} metric for ordered categories, which is often used to evaluate AS methods \cite{naepchal}. 


\subsection{Experimental setting}
\label{setting}

In the quantitative experiment, we focus on studying on whether adding scorer information leads to improved AS accuracy. Therefore, when we are splitting dataset into training, validation, and test sets, we ensure that every scorer is included in the training set. We divide the data points (question-response pairs, scorer ID, score) into $10$ equally-sized folds for cross validation. 
%We ensure that each fold contains enough data cover all of the scorers. 
During training, we use $8$ folds as training data, $1$ fold for validation for model selection, and $1$ fold for the final testing to evaluate the AS models. 

For fair comparison, every model uses BERT\footnote{\url{https://huggingface.co/bert-base-uncased}} as the pre-trained model for question-response pair representation, which has been shown to result in state-of-the-art AS accuracy in prior work~\cite{edm22}. We emphasize that our work on \textbf{scorer models} can be added on top of \textbf{any} AS method for response representation; applying these models on other AS methods is left for future work. We use the Adam optimizer, a batch size of $16$, a learning rate of $1e-5$ for $10$ training epochs on an NVIDIA RTX$8000$ GPU. We do not perform any hyper-parameter tuning and simply use the default settings. 

% \begin{table}[]
% \begin{tabularx}{0.6\textwidth}{X|l|l|l}
% \hline
%                                                              & AUC   & RMSE  & Kappa \\ \hline
% Universal Classification                                     & 0.752 & 0.959 & 0.609 \\ \hline
% Unordered Categorical Classification with teacher embedding& 0.763 & 0.933 & 0.618 \\ \hline
% Ordered Categorical Classification with teacher information (ordinal log-loss)& 0.765 & 0.922 & 0.622 \\ \hline
% Ordered Categorical Classification with teacher information (mse loss)& 0.767 & 0.909 & 0.618 \\ \hline
% Unordered Categorical Classification with teacher information conditioning on [CLS]&0.771 & 0.944 & 0.634 \\\hline
% Unordered Categorical Classification with teacher information with different classification head&0.766 & 0.943 & 0.626 \\\hline
% Ordered Categorical Classification with teacher information conditioning on [CLS](oll)&0.775 & 0.933 & 0.637 \\\hline
% %Unordered Categorical Classification with teacher information& 0.766 & 0.943 & 0.626 \\ \hline
% %Ordered Categorical Classification with teacher information (bin boundary setting)& 0.726 & 1.054 & 0.563 \\ \hline
% %Ordered Categorical Classification with teacher information (ordinal log-loss)& 0.770 & 0.954 & 0.626 \\ \hline
% %Regression with teacher information& 0.762 & 0.947 & 0.624 \\ \hline
% %Universal Head Classification with Addition of Teacher embed & 0.762 & 0.957 & 0.617 \\ \hline \hline  #temperature = 1
% %Unordered Categorical Classification with teacher information conditioning on response embedding&0.755  & 1.027 & 0.595 \\ \hline
% \end{tabularx}
% \caption{Comparing different scorer models on short-answer math scoring. The combination of response-dependent bias and variance with the OLL loss outperforms other scorer models and training losses. \ml{is it possible to add some standard deviation values?} \ml{we need better names for these methods}}
% \end{table}

\begin{table*}[]
\begin{tabular}{l|l|l|l|l}
\hline
Bias ($b$) \& Temperature ($\alpha$) & Loss Function & AUC & RMSE & Kappa \\ \hline
Universal ($b_c$, $\alpha$ = 1)  & CE            & 0.765 $\pm$ 0.003    &0.954 $\pm$ 0.014      & 0.614 $\pm$ 0.009      \\ \hline
Universal ($b_c$, $\alpha$ = 1)  & MSE            & 0.764 $\pm$ 0.003    &0.946 $\pm$ 0.018      & 0.615 $\pm$ 0.008      \\ \hline
Universal ($b_c$, $\alpha$ = 1)  & OLL            & 0.768 $\pm$ 0.003    &0.944 $\pm$ 0.015      & 0.617 $\pm$ 0.006      \\ \hline
Scorer-specific ($b_{c,j}$, $\alpha_j$)      & CE            & 0.768 $\pm$ 0.005    &   0.928 $\pm$ 0.023   &   0.628 $\pm$ 0.006    \\ \hline
Scorer-specific  ($b_{c,j}$, $\alpha_j$)        & MSE    &  0.772 $\pm$ 0.005   &  0.926 $\pm$ 0.025    &  0.625  $\pm$  0.006  \\ \hline
Scorer-specific   ($b_{c,j}$, $\alpha_j$)       & OLL           &  0.770 $\pm$ 0.003   &   \textbf{0.916 $\pm$ 0.013}   &  0.628 $\pm$ 0.004     \\ \hline
Content-driven ($b_{c,j}(\mathbf{r}_i)$, $\alpha_j(\mathbf{r}_i)$)        & CE            &    0.772 $\pm$ 0.003  & 0.923 $\pm$ 0.016     &  0.631 $\pm$ 0.006      \\ \hline
Content-driven ($b_{c,j}(\mathbf{r}_i)$, $\alpha_j(\mathbf{r}_i)$)        & MSE            &    0.774 $\pm$ 0.004 &   0.922 $\pm$ 0.021   & 0.629 $\pm$ 0.005      \\ \hline
Content-driven ($b_{c,j}(\mathbf{r}_i)$, $\alpha_j(\mathbf{r}_i)$)       & OLL           &   \textbf{0.779 $\pm$ 0.004}  &  0.924 $\pm$ 0.013    &    \textbf{0.641 $\pm$ 0.005}   \\ \hline
\end{tabular}
\vspace{.2cm}
\caption{Comparing different scorer models on short-answer math scoring. The combination of content-driven scorer bias and temperature with the OLL loss outperforms other scorer models and training losses.}
\label{tab:as}
\end{table*}

\subsection{Results and discussion}
\label{result}

Table~\ref{tab:as} shows the mean and standard deviation of each scorer model trained under each loss function. We see that generally, models with content-driven scorer biases and variances outperform scorer-specific biases and variances, which outperform the base AS model that treats each scorer the same with universal values for bias and variance. The improvement in AS accuracy is significant, up to about $0.02$ in the most important metric--Kappa, for the content-driven biases and variances over the standard AS approach of not using scorer information. This observation validates the need to account for individual scorer preferences and tendencies in the highly subjective AS task. Meanwhile, since the content-driven scorer bias and variance models outperform the scorer-specific bias and variance models, we can conclude that the content of the question and response does play an important role in scorer preference. 

We also observe that training scorer models with the OLL loss outperforms the other losse, while training with the MSE loss does not even lead to the best results on the RMSE metric. This observation suggests that taking into account the ordered nature of score categories instead of treating them as parallel ones is important to the AS task. 

